Multi-view 3D Reconstruction of a Texture-less Smooth Surface of Unknown Generic Reflectance

Recovering the 3D geometry of a purely texture-less object with generally unknown surface reflectance (e.g. non-Lambertian) is regarded as a challenging task in multi-view reconstruction. The major obstacle revolves around establishing cross-view correspondences where photometric constancy is violated. This paper proposes a simple and practical solution to overcome this challenge based on a co-located camera-light scanner device. Unlike existing solutions, we do not explicitly solve for correspondence. Instead, we argue the problem is generally well-posed by multi-view geometrical and photometric constraints, and can be solved from a small number of input views. We formulate the reconstruction task as a joint energy minimization over the surface geometry and reflectance. Despite this energy is highly non-convex, we develop an optimization algorithm that robustly recovers globally optimal shape and reflectance even from a random initialization. Extensive experiments on both simulated and real data have validated our method, and possible future extensions are discussed.

==> figure_convergence_detail.tex <==
\begin{figure}
    \centering
\begin{python}
it_nos = ['00', '01', '04', '09', '29']
brdf_strs = ['gold-metallic-paint', 'grease-covered-steel']
for brdf_str in brdf_strs:
    print r'\\' + brdf_str + r'\\'
    for i,s in enumerate(it_nos):
        print r"\begin{subfigure}[b]{0.09\textwidth}\centering\vspace*{-0cm}\hspace*{-0.4cm} \includegraphics[width=1.115\textwidth]{img/%s-1d-bunny-%s-hist-a.eps}\\\vspace*{-0.05cm}\hspace*{-0.4cm} \includegraphics[width=1.115\textwidth]{img/%s-1d-bunny-%s-hist-d.eps}\\\vspace*{-0.05cm}\hspace*{-0.2cm}\includegraphics[width=1.115\textwidth]{img/%s-1d-bunny-%s-f.eps}\caption*{%s}\end{subfigure}" % (brdf_str,s,brdf_str,s,brdf_str,s,'it. {}'.format(str(int(s)+1)))
\end{python}
    \caption{Angular errors histogram, depth error histogram, and BRDF scattered plot at the 1st, 2nd, 5th, 10th and 30th iteration.}
    \label{fig:figure_convergence_detail}
\end{figure}

==> figure_convergence_overview.tex <==
\begin{figure}
    \centering
\begin{python}
brdf_strs = ['brass', 'grease-covered-steel']
height = '1.5'
print r"\begin{subfigure}[b]{0.09\textwidth}\centering"
for i,s in enumerate(brdf_strs):
    print r"\hspace*{-1cm}\includegraphics[height=%scm]{img/%s-1d-bunny-brdf-mae.eps}\\" % (height, s)
print r"\caption*{BRDF err}\end{subfigure}"
print r"\begin{subfigure}[b]{0.09\textwidth}\centering"
for i,s in enumerate(brdf_strs):
    print r"\hspace*{-0.5cm}\includegraphics[height=%scm]{img/%s-1d-bunny-depth-rms.eps}\\" % (height, s)
print r"\caption*{depth err}\end{subfigure}"
print r"\begin{subfigure}[b]{0.09\textwidth}\centering"
for i,s in enumerate(brdf_strs):
    print r"\hspace*{-0cm}\includegraphics[height=%scm]{img/%s-1d-bunny-normal-mean.eps}\\"% (height, s)
print r"\caption*{normal err}\end{subfigure}"
print r"\begin{subfigure}[b]{0.09\textwidth}\centering"
for i,s in enumerate(brdf_strs):
    print r"\hspace*{0.2cm}\includegraphics[height=%scm]{img/%s-1d-bunny-photometric-loss.eps}\\" % (height, s)
print r"\caption*{$L_p$}\end{subfigure}"
print r"\begin{subfigure}[b]{0.09\textwidth}\centering"
for i,s in enumerate(brdf_strs):
    print r"\hspace*{0.2cm}\includegraphics[height=%scm]{img/%s-1d-bunny-brdf.eps}\\" % (height, s)
print r"\caption*{$L_p$}\end{subfigure}"
\end{python}
\caption{Error convergence plot vs. iterations}
\label{fig:figure_convergence_overview}
\end{figure}

==> figure_material.tex <==
\begin{figure}
    \centering
\begin{python}
brdf_strs = ['brass'] * 10
for i,s in enumerate(brdf_strs):
    print r"\begin{subfigure}[b]{0.09\textwidth}\centering\includegraphics[width=\textwidth,angle=180,origin=c]{img/%s-1d-bunny-00-r.png}\\\vspace*{-0cm}\hspace*{-0.4cm} \includegraphics[width=1.115\textwidth]{img/%s.eps}\\\vspace*{-0.05cm}\hspace*{-0.4cm} \includegraphics[width=1.3\textwidth]{img/%s_2d.eps}\caption*{%s}\end{subfigure}" % (s,s,s,s)
    if i % 5 == 4:
        print r"\\"
\end{python}
    \caption{Materials used for rendering, from top to bottom, example rendered bunny model, 1d brdf, 2d brdf slice}
    \label{fig:figure_shape}
\end{figure}

==> figure_shape.tex <==


\begin{figure}
    \centering
\begin{python}
model_strs = ['bunny'] * 12
for i,s in enumerate(model_strs):
    print r"\begin{subfigure}[b]{0.11\textwidth}\centering\includegraphics[width=\textwidth,angle=180,origin=c]{img/brass-1d-%s-00-gtn.png}\caption*{%s}\end{subfigure}" % (s,s)
    if i % 4 == 3:
        print r"\\"
\end{python}
    \caption{Models used for rendering}
    \label{fig:figure_shape}
\end{figure}

==> figure_visual_results.tex <==
\begin{figure}
    \centering
\begin{python}
model_strs = ['bunny'] * 12
for i,s in enumerate(model_strs):
    print r"\begin{subfigure}[b]{0.11\textwidth}\centering\includegraphics[width=\textwidth,angle=180,origin=c]{img/brass-1d-%s-00-gtn.png}\caption*{%s}\end{subfigure}" % (s,s)
    if i % 4 == 3:
        print r"\\"
\end{python}
    \caption{Models used for rendering}
    \label{fig:figure_shape}
\end{figure}

==> macros3.tex <==
%\input{local-definitions}
\newcommand{\tr}{\mbox{$^{\top}$}}
\newcommand{\trinv}{\mbox{$^{\top\,-1}$}}
\newcommand{\mtr}{\mbox{$^{-\top}$}}
\newcommand{\rank}{\mbox{\rm rank}}
\newcommand{\sign}{\mbox{\rm sign}}
\newcommand{\diag}{\mbox{\rm diag}}
\newcommand{\med}{\mbox{\rm med}} % maybe change/drop this
\newcommand{\adj}{\mbox{$^*$}}
\def\ijk{_i^{jk}}
\def\uvw{_u^{vw}}
\def\Tri{{\cal T}}
\def\Tijk{\Tri\ijk}
\def\Tuvw{\Tri\uvw}

% Real, complex numbers and integers
% \newcommand{\R}{{\cal R}}
% \newcommand{\C}{{\cal C}}
\def\R{{\rm I} \! {\rm R}} 
\def\C{{\rm l} \! \! \! {\rm C}}
\def\ints{{\rm Z} \! \! {\rm Z}}


% Standardized references
\newcommand{\app}[1]{appendix~\ref{app:#1}}
\newcommand{\App}[1]{Appendix~\ref{app:#1}}
\newcommand{\eq}[1]{(\ref{eq:#1})}
\newcommand{\eqn}[1]{(\ref{eq:#1})}
\newcommand{\fig}[1]{Fig~\ref{fig:#1}}
\newcommand{\tab}[1]{table~\ref{tab:#1}}
\newcommand{\Tab}[1]{Table~\ref{tab:#1}}
\newcommand{\sect}[1]{section~\ref{sec:#1}}
\newcommand{\ch}[1]{chapter~\ref{ch:#1}}
\newcommand{\Ch}[1]{Chapter~\ref{ch:#1}}
\newcommand{\thm}[1]{Theorem~\ref{thm:#1}}

\newcommand{\num}[1]{(~\ref{num:#1})}
\newcommand{\Thm}[1]{Theorem~\ref{thm:#1}}
\newcommand{\pro}[1]{Proposition~\ref{pro:#1}}
\newcommand{\cor}[1]{Corollary~\ref{cor:#1}}
\newcommand{\Pro}[1]{Proposition~\ref{pro:#1}}
\newcommand{\defn}[1]{definition~\ref{def:#1}}
\newcommand{\algo}[1]{table~\ref{alg:#1}}
\newcommand{\lem}[1]{lemma~\ref{lem:#1}}

\newcommand{\SKIP}[1]{} % Used to skip stuff we do not want type-set

%
\newcommand{\vv}[2]
   {\mbox{$
      \left(
         \begin{array}{c}
         #1 \\ #2
         \end{array}
      \right )
   $}}
%
\newcommand{\vvv}[3]
   {\mbox{$
      \left(
         \begin{array}{c}
         #1 \\ #2 \\ #3
         \end{array}
      \right )
   $}}
%
\newcommand{\vvvv}[4]
   {\mbox{$
      \left(
         \begin{array}{c}
         #1 \\ #2 \\ #3 \\ #4
         \end{array}
      \right )
   $}}
%
\newcommand{\vm}[2]
   {\mbox{$
      \left[
         \begin{array}{c}
         #1 \\ #2
         \end{array}
      \right ]
   $}}
%
\newcommand{\vvm}[3]
   {\mbox{$
      \left[
         \begin{array}{c}
         #1 \\ #2 \\ #3
         \end{array}
      \right ]
   $}}
%
\newcommand{\vvvm}[4]
   {\mbox{$
      \left[
         \begin{array}{c}
         #1 \\ #2 \\ #3 \\ #4
         \end{array}
      \right ]
   $}}
%
\newcommand{\mm}[4]
   {\mbox{$
      \left[
         \begin{array}{ccc}
         #1 & #2    \\
         #3 & #4 
         \end{array}
      \right]
   $}}
%
\newcommand{\mmm}[9]
   {\mbox{$
      \left[
         \begin{array}{ccc}
         #1 & #2 & #3   \\
         #4 & #5 & #6   \\
         #7 & #8 & #9
         \end{array}
      \right]
   $}}

%
% Quick way to do matrices
\newcommand{\mbegin} {\left [ \begin{array}}
\newcommand{\mstart} {\mbegin}
\newcommand{\mc}     {\mbegin{c}}
\newcommand{\mcc}    {\mbegin{cc}}
\newcommand{\mccc}   {\mbegin{ccc}}
\newcommand{\mcccc}  {\mbegin{cccc}}
\newcommand{\mccccc} {\mbegin{ccccc}}
\newcommand{\mend}   {\end{array} \right ]}

\newcommand{\detbegin} {\left | \begin{array}}
\newcommand{\detend}   {\end{array} \right |}

% Same for vectors
\newcommand{\vbegin} {\left ( \begin{array}{c}}
\newcommand{\vstart} {\vbegin}
\newcommand{\vend} {\end{array}\right )}

%
%
%
\newcommand{\lra}{\leftrightarrow}
\newcommand{\Po}{\mbox{\({\cal P}^1\)}}
\newcommand{\PP}{\mbox{\({\cal P}^2\)}}
\newcommand{\PPP}{\mbox{\({\cal P}^3\)}}
\newcommand{\PPPPP}{\mbox{\({\cal P}^5\)}}
\newcommand{\Pn}{\mbox{\({\cal P}^n\)}}
\newcommand{\sk}[1]{[#1]_\times}
\newcommand{\bm}[1]{\mbox{\bf $#1$}}
%

% Stuff for doing the qed sign.
\def\squareforqed{\hbox{\rlap{$\sqcap$}$\sqcup$}}

\def\qed{\ifmmode\squareforqed\else{\unskip\nobreak\hfil
	\penalty50\hskip1em\null\nobreak\hfil\squareforqed
	\parfillskip=0pt\finalhyphendemerits=0\endgraf}\fi}

% Stuff for doing vector. NB need to not use small for lower case.
\def\vecs#1{\mathchoice%
	{\mbox{\bf \small $\displaystyle\bf#1$}}
	{\mbox{\bf \small $\textstyle\bf#1$}}
	{\mbox{\bf \small $\scriptstyle\bf#1$}}
	{\mbox{\bf \small $\scriptscriptstyle\bf#1$}}}
\def\vs#1{\protect\vecs #1}

\def\vec#1{\mathchoice%
	{\mbox{\bf $\displaystyle\bf#1$}}
	{\mbox{\bf $\textstyle\bf#1$}}
	{\mbox{\bf $\scriptstyle\bf#1$}}
	{\mbox{\bf $\scriptscriptstyle\bf#1$}}}
\def\v#1{\protect\vec #1}

% Stuff for making labels visible
\newcommand{\showlabel}[1]
	{\hskip 0.0em\marginpar{\quad\fbox{\scriptsize\rm#1}}}

\newcommand{\showeqnlabel}{
	\hbox to 0pt{\quad\quad\relax\fbox{\scriptsize\rm\eqnlblx}%
	\gdef\eqnlblx{xxxx}}} \newcommand{\eqnlblx}{}

\def\@eqnnum{\rm (\theequation)\showeqnlabel}

\newcommand{\eqnlabel}[1]{\protect\label{#1}\gdef\eqnlblx{#1}}

\newcommand{\mylabel}[1]{\label{#1}\showlabel{#1}}

\newcommand{\nofig}[1]{\centerline{\bf Figure here}}

% Stuff for doing matrix.
\def\mat#1{\mathchoice{\mbox{\bf$\displaystyle\tt#1$}}
	{\mbox{\bf$\textstyle\tt#1$}}
	{\mbox{\bf$\scriptstyle\tt#1$}}
	{\mbox{\bf$\scriptscriptstyle\tt#1$}}}
\def\m#1{\protect\mat #1}

%\newcommand{\matx}[1]{{\tt #1}}
\newcommand{\matx}[1]{{\m #1}}
